Revisiting DocRED -- Addressing the False Negative Problem in Relation Extraction

The DocRED dataset is one of the most popular and widely used benchmarks for document-level relation extraction (RE). It adopts a recommend-revise annotation scheme so as to have a large-scale annotated dataset. However, we find that the annotation of DocRED is incomplete, i.e., false negative samples are prevalent. We analyze the causes and effects of the overwhelming false negative problem in the DocRED dataset. To address the shortcoming, we re-annotate 4,053 documents in the DocRED dataset by adding the missed relation triples back to the original DocRED. We name our revised DocRED dataset Re-DocRED. We conduct extensive experiments with state-of-the-art neural models on both datasets, and the experimental results show that the models trained and evaluated on our Re-DocRED achieve performance improvements of around 13 F1 points. Moreover, we conduct a comprehensive analysis to identify the potential areas for further improvement. Our dataset is publicly available at https://github.com/tonytan48/Re-DocRED.

==> EMNLP_2022/sections/1_introduction.tex <==
\section{Introduction}
The field of relation extraction (RE) is related to knowledge bases (KBs). Most popular relation extraction datasets are constructed from knowledge triples in KBs. For example, the TACRED dataset~\citep{zhang-etal-2017-position} is constructed by the TAC Knowledge Base Population challenge. The NYT10 \citep{riedel-etal-2013-relation} dataset matched the Freebase Knowledge base \citep{bollacker2008freebase} to the New York Times corpus \citep{sandhaus2008new}. Wiki20~\citep{gao2021manual} and DocRED~\citep{yao2019docred} originated from distant supervision from the Wikidata knowledge base~\citep{vrandevcic2014wikidata} and Wikipedia articles. 
% During the dataset production process of distant supervision, 
By exploiting distant supervision, relation triple candidates can be retrieved from the knowledge bases for a given piece of text. 
The retrieved triples are based on entity co-occurrence only, and they may not be related to the context. This is known as the false positive (FP) problem (\citealp{bing-etal-2015-improving}; \citealp{xiao-etal-2020-denoising}). 
\begin{figure}[!t]
\centering{
\small{
\begin{tabular}{|p{0.92\columnwidth}|}
\hline
\vspace{-.1cm}
"\textbf{I Knew You Were Trouble}~" is a song recorded by American singer - songwriter \textbf{Taylor Swift} for her fourth studio album , \textbf{Red} ( 2012 ) . It was released on \textbf{October 9 , 2012} , in \textbf{the United States} by \textbf{Big Machine Records} as the third promotional single from the album . Later , " \textbf{I Knew You Were Trouble} " was released as the third single from \textbf{Red} on \textbf{November 27 , 2012} , in \textbf{the United States }. It was written by \textbf{Swift} , \textbf{Max Martin} and \textbf{Shellback} , \colorbox{LightYellow}{\underline{with the production handled by the latter two}} ... It later peaked at number two in \textbf{January 2013} , blocked from the top spot by \textbf{Bruno Mars}’ " \textbf{Locked Out of Heaven} " . At the inaugural \textbf{YouTube Music Awards }in 2013 , " \textbf{I Knew You Were Trouble }" won the award for \textbf{YouTube} phenomenon …  \\
\vspace{0.05cm}
\textcolor{orange}{\textbf{DocRED}}: (\textbf{I Knew You Were Trouble}, \textit{producer}, \textbf{Max Martin}); (\textbf{Taylor Swift},~\textit{country of citizenship},~ \textbf{the United States}) ...  \\
\vspace{0.05cm}
\textcolor{skyblue}{\textbf{Re-DocRED}}:  (\textbf{I Knew You Were Trouble}, \textit{producer}, \textbf{Max Martin}); (\textbf{I Knew You Were Trouble},~\textit{producer},~\textbf{Shellback}) ... 
\vspace{.1cm}
\\
\hline
% \vspace{-.1cm}
\end{tabular}
}}
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{-0pt}
\caption{A sample document in our Re-DocRED dataset. From the \colorbox{LightYellow}{\underline{highlighted evidence}}, it can be inferred that ``I Knew You Were Trouble'' was produced by both ``Max Martin'' and ``Shellback'', but in the previous incomplete DocRED dataset, only the first producer is labeled.}
\label{fig:example-doc}
\end{figure}

% , which is to correct existing annotations~(\citealp{yao2019docred}; \citealp{alt2020tacred}).
% During the dataset production process, most existing works only focused on the discussion of reducing false positives, which is to discard the relation triples that are not related to the context.

However, the false negative (FN) problem in the relation extraction datasets receives less attention as compared to FPs. Without resolving this issue, the annotations of the datasets are incomplete.
% However, the false negative problem in the relation extraction datasets is overlooked.
Recent efforts on addressing the false negative problem are from the model perspective (\citealp{chen2021h}; \citealp{hao-etal-2021-knowing}), which aim to denoise the false negative data during training.
The challenge for these approaches is that both development and test sets can be incomplete at the same time. Without a completely annotated dataset, the current evaluation is ill-defined.
% , but the incomplete annotations can exist in the evaluation dataset as well. If the evaluation dataset is incomplete, it will penalize the factually correct triples during evaluation, which makes the relation extraction problem ill-defined. 
% For example, in Figure~\ref{fig:example-doc}, the article reflects that the song ``I Knew You Were Trouble'' was produced by both ``Max Martin'' and ``Shellback'', but ``Shellback'' is not included in the DocRED dataset. 
% For example, in Figure~\ref{fig:example-doc}, the article reflects that the song \textbf{I Knew You Were Trouble} was produced by both \textbf{Max Martin} and \textbf{Shellback}, but only \textbf{Max Martin} as the producer in the DocRED dataset. 
% The problem of incompleteness in the DocRED dataset can be originated from two causes: 1) The incompleteness in the Wikidata knowledge base and 2) DocRED relies on an LSTM-based relation extraction model to generate candidates for human annotators, which may be insufficient.
% Due to strong digital sales , the song debuted at number three on the \textbf{Billboard Hot 100} chart in \textbf{the United States} , selling more than 416,000 ~ copies within its first week ;\textbf{}

%\textbf{False Positive}: (\textbf{Bruno Mars},~ \textbf{the United States},~ \textit{country of citizenship}) 
% The relation extraction task is highly difficult, and it is partially due to the existing benchmark datasets are flawed. 

Several re-annotation works revised the existing sentence-level relation extraction datasets. 
\citet{alt2020tacred} re-annotated a small amount of challenging samples in the development and test sets of the TACRED dataset \citep{zhang-etal-2017-position}. \citet{stoica2021re} extended this work and re-annotated the training, development, and test sets of TACRED with a semantically refined label space. Besides, \citet{gao2021manual} re-annotated the test sets of two distantly supervised RE datasets. 
Even though their discussions and examples emphasized the efforts on correcting the false positive samples, all
the revised versions of the datasets have a significant increase of positive samples. 
That is, many samples that are previously labeled as \textit{no\_relation}~(NA) are re-annotated with relation labels in the revised datasets.
We show the detailed statistics in Table~\ref{tab:data-stats}, which indicates that the false negative problem is prevalent in the sentence-level relation extraction field. 
% We can also observe that the total number of triples in the revised datasets increases 
%\textcolor{red}{NA stands for? how do you calculate it, will need to include it  in the footnote or appendix.}
% This observation shows there are considerable amount of negative instances that are relabeled as positive instances, showing that the false negative problem is prevalent in the sentence-level relation extraction field. 
Compared to the sentence-level task, document-level RE is more susceptible to the false negative problem. This is primarily because document-level RE involves significantly more entity pairs in a raw text, as shown in Table \ref{tab:data-stats}. 
Note that the objective of the RE task is to determine the relation types for all entity pairs, and the number of entity pairs is quadratic in the number of entities.

In this paper, we address the false negative problem in DocRED. We find that the false negative problem arises due to two reasons. 
First, although the Wikidata knowledge base provides a good starting point for distantly supervised annotation of DocRED, it is highly sparse and far from complete. There are many relation triples that are 
% reflected in the Wikipedia articles but 
not in the Wikidata KB. 
For example, in Figure~\ref{fig:example-doc}, the article reflects that the song ``I Knew You Were Trouble'' was produced by both ``Max Martin'' and ``Shellback'', but the fact that ``Shellback'' is the other producer is not included in both the knowledge base and the DocRED dataset. 
Second, the additional relation triples recommended by the RE model and human annotators cannot cover the ground-truth relation triples that are missed from the Wikidata. A detailed discussion is given in Section \ref{sec:preliminaries}. 
With the incompletely annotated development and test sets, the previous evaluation does not necessarily provide a fair reference.
Therefore, we propose to revise the DocRED dataset to recover the incomplete annotations through an iterative approach with human in the loop.
Specifically, we use multiple state-of-the-art document-level RE models to generate relation candidates and ask human annotators to examine the recommended triples. The details of our iterative human-in-the-loop annotation process are given in Section \ref{sec:revision}.

%This part shall be expanded in detail, not only does Huang2022DoesRP miss certain triples, it is also not as precise as ours. 
Most recently, \citet{Huang2022DoesRP} also identify the false negative issue in DocRED \cite{yao2019docred}. They combat the problem by annotating 96 documents from scratch with two expert annotators. 
However, annotating relation triples from scratch is different from revising recommended triples, and it is difficult to scale up to a dataset of a larger size.
We provide a comprehensive analysis between our approach and the annotating-from-scratch approach in Appendix \ref{app:comparisonwithscratch}.
Compared to \citet{Huang2022DoesRP}, our approach is better in the following aspects. First, our dataset is significantly larger in size (4,053 vs 96 documents). 
Second, the precision of our annotation is higher. 
Third, our evaluation dataset contains more triples per document than \citet{Huang2022DoesRP}, indicating that our dataset better tackles the incompleteness problem of DocRED. 
Fourth, our dataset annotation approach is more scalable and can be extended to an arbitrary number of relation types. 
%Although their annotation contains more number of triples, we find that the dataset still have missing triples.
% Although human annotators are asked to supplement the omitted triples, it is challenging to annotate the triples from scratch \cite{}. We find that the number of human-supplied triples is limited, and detailed discussion can be found in Section \ref{sec:preliminaries}. 
% Therefore, we revise the DocRED dataset to alleviate the false negative problem.

Our contributions can be summarized as follows:
\begin{itemize}
    \item We identify the overwhelming false negative problem in relation extraction. 
    \item We show that the false negative problem is the cause of performance bottleneck on many relation extraction datasets, and we also provide a high-quality revised version of the document-level relation extraction dataset Re-DocRED. 
    \item Moreover, we conduct comprehensive experimental analysis to identify the potential areas for further improvement.
\end{itemize}

\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{lccccccl} 
\toprule
\textbf{Dataset}            & \multicolumn{1}{c}{\textbf{\# Relations}} & \multicolumn{1}{c}{\textbf{\# Triples}} & \multicolumn{1}{c}{\textbf{\# Samples}} & \multicolumn{1}{c}{\textbf{Avg. \# Words}} & \multicolumn{1}{c}{\textbf{Avg. \# Entities}} & \multicolumn{1}{c}{\textbf{Avg. \# Entity Pairs}} & \multicolumn{1}{c}{\textbf{NA}}  
\\ 
\midrule
\multicolumn{2}{l}{\textbf{Sentence-level}} \vspace{0.05cm} \\ 
Wiki20~\citep{han-etal-2020-data}     & 454                             & 15,026                        & 28,897                       & 25.7                             & 2                                   & 1                                       & 48.0\%                 \\
Wiki20m~\citep{gao2021manual} & 81                              & 103,709                       & 137,986                      & 25.6                             & 2                                   & 1                                       & 24.8\%{\color{green}$\downarrow$}                 \\
TACRED~\citep{zhang-etal-2017-position}     & 42                              & 21,373                        & 106,264                      & 36.4                             & 2                                   & 1                                       & 79.9\%                 \\
Re-TACRED~\citep{stoica2021re}  & 40                              & 33,690                        & 91,467                       & 36.4                             & 2                                   & 1                                       & 63.2\%{\color{green}$\downarrow$} \\ 
\midrule
\multicolumn{2}{l}{\textbf{Document-level}} \vspace{0.05cm} \\
HacRED~\citep{cheng-etal-2021-hacred}     & 26                              & 56,798                        & 7,731\tnote{1}                      & 122.6                            & 10.7                                & 163.9                                   & 95.7\%                 \\
DocRED~\citep{yao2019docred}     & 96                              & 50,503                        & 4,053\tnote{1}                        & 198.4                            & 19.5                                & 393.6                                  & 97.1\%                 \\
\textbf{Re-DocRED} (Ours)  & 96                              & 120,664                       & 4,053                        & 198.4                            & 19.4\tnote{2}                            & 391.0                                  & 94.0\%{\color{green}$\downarrow$}                  \\
\bottomrule
\end{tabular}
  \begin{tablenotes}[para]
    \item[1] We do not include the blind test sets for these two datasets.  \item[2] We also resolve the coreferential errors. Details are given in Appendix~\ref{app:coreference}.
    % \vspace{-0.3cm}
  \end{tablenotes}
\end{threeparttable}
}
% \setlength{\abovecaptionskip}{1pt}
% \setlength{\belowcaptionskip}{-2pt}
\caption{Statistics of relation extraction datasets. We can see that all re-annotation efforts on sentence-level relation extraction datasets (Wiki20 $\rightarrow$ Wiki20m, TACRED $\rightarrow$ Re-TACRED) result in significantly smaller percentages of \textit{no\_relation} (NA) samples, indicating that false negative is a common problem in the RE datasets.}
% The Wiki20m dataset is the revised version of the Wiki20 dataset, where the test set is re-annotated manually. The Re-TACRED dataset is a re-annotated version of the TACRED dataset.
%\textcolor{red}{qingyu: solve the mentioned problems in the footnote}
%\textcolor{red}{will edit the stats and modify the lines 43-50 in the intro and section 2.3.}
\label{tab:data-stats}
\end{table*}
%\footnote{We also corrected the coreferential errors in DocRED, leading to a a smaller number of entities.}  

==> EMNLP_2022/sections/2_preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
\subsection{Background of the DocRED Dataset}
\label{sec:background-docred}
The DocRED dataset~\citep{yao2019docred} is one of the popular and widely-studied benchmark datasets for document-level relation extraction. 
% It consists of two portions: distantly supervised (DS) data and human-annotated data.
% The first portion contains 101,873 Wikipedia articles with distantly supervised relation triples. The distantly supervised documents are created by mapping the relation triples in the Wikidata database to the Wikipedia articles. That is to say, as long as two entities co-occur in the same document, all the relations between these two entities in the Wikidata knowledge base will be mapped to this document. 
% For example, the sentence ``Barack Obama was born in the United States.'' only reflects (``Barack Obama'', \textit{born in}, ``the United States''), whereas distant supervision will map (``Barack Obama'', \textit{head of government}, ``the United States'') to this sentence based on triples in the knowledge base. 
% Therefore, the relation triples that are extracted by the DS data are noisy in nature. 
% The first portion contains 101,873 Wikipedia articles with distantly supervised relation triples. The distantly supervised documents are created by mapping the relation triples in the Wikidata database to the Wikipedia articles. That is to say, as long as two entities co-occurred in the same article, all the relations between these two entities in the Wikidata knowledge base will be mapped to this article. For example, the sentence ``Barack Obama was born in the United States.'' only reflects (\textbf{Barack Obama}, \textit{born in}, \textbf{the United States}), whereas distant supervision will map (\textbf{Barack Obama}, \textit{head of government}, \textbf{the United States}) to this sentence based on triples in the knowledge base. Therefore, the distantly supervised data is noisy in nature. 
% The second portion of t
The dataset contains 5,053 Wikipedia documents, where each document has an average length of 196.7 words, and an average of 19.5 entities.
With 97 predefined relation types (including \textit{no\_relation}) and an average of 393.6 entity pairs, there exist around 38,000 relation triple candidates per document to be annotated.
To reduce the annotation workload, a recommend-revise scheme is adopted.
Specifically, relation triple candidates are recommended from distantly supervised data and predictions of an RE model.
On average for each document, 19.9 triples are suggested from distantly supervised data and 7.8 triples are recommended by relation extraction models. Human annotators are asked to read the documents and review the relation triple candidates, and wrong recommendations will be discarded. As a result, an average of 12.5 triples per document are kept in the DocRED dataset.


%Based on the final reported statistics, 57.2\% of relation triples from distant labeling and 48.2\% from RE models are annotated as correct.Besides filtering the wrong relation triples, human annotators are asked to add the omitted ones. However, we find that it is  challenging\footnote{By computing their reported statistics, the sum of the revised triples is 15.1 per document, which is already more than the reported average number of triples (12.5) in the DocRED dataset.} to add the omitted relation triples, and it can be inferred that the annotators of the DocRED dataset mainly filtered out the false positive triples. 

%\bing{\cchar{也就是distantly labeling？}}
%\bing{\cchar{不是annotated，应该是confirm为正确？}}
%\bing{\cchar{没懂在讲什么。是filter掉15.1？还是保留的是15.1？是19.9*57.2\%+7.8*48.2\%吧?}}
% However, by computing their reported statistics, the sum of the filtered triples is 15.14 per document, which is quite different from the reported average number of triples in the training and development set, 12.53 and 12.33, respectively.
% It is doubtful that the annotators have supplemented the omitted ones, because from the statistics, 57.2\% relation instances from entity linking and 48.2\% from RE models are reserved. The sum of the filtered triples is 15.14 per document if we compute by their reported numbers. But the average number of triples in the training and development set are 12.53 and 12.33, respectively. 
% Hence, it can be inferred that the annotators of the DocRED dataset mainly filtered out the incorrect triples, and it is challenging to supplement the omitted ones that are different from distantly supervised triples and the recommendations from the RE model. 


% It is worthwhile to notice that the construction procedures of the DocRED dataset relies on a strong bias, which is the combination of the recommended triples from the RE model and the distantly supervised triples almost contains all the relation instances in the raw articles. 
% This bias is not true since the relations in Wikidata knowledge base are sparse and incomplete. Furthermore, the recommended triples from the RE model are  not enough for covering the remaining ground truth triples.
% In our empirical analysis based on the top-performing models on the DocRED leaderboard, many predicted triples are correct but are not annotated in the DocRED dataset. Therefore, it is important to review the dataset and to identify the true bottleneck of the document-level RE task. 

% In our empirical analysis from the top-performing models on the DocRED leaderboard, there are many triples from the model predictions that are correct triples but are not annotated in the DocRED dataset. Therefore, it is important to review the dataset and to identify the true bottleneck of the document-level RE task. 




\subsection{Problem of Incomplete Annotation}
\label{sec:problem-docred}
Based on our empirical analysis of the top-performing models \cite{tan2022document, zhang2021document, zhou2021document} on the DocRED leaderboard, many predicted triples are correct but are not annotated in the DocRED dataset. Therefore, it is important to review the dataset and identify the true bottleneck of document-level RE. We identify incomplete annotation as the major issue in the DocRED dataset. As mentioned in Section~\ref{sec:background-docred}, it is difficult to annotate a document-level RE dataset from scratch. The DocRED dataset is mainly created by human filtering the recommended relation triples in distantly supervised data and predictions from an RE model.
It is worth noting that the construction procedure of DocRED relies on the underlying assumption that the combination of the recommended triples by distant supervision and the RE model contains almost all the ground-truth relation triples in the documents. 
This assumption is not true since the relations in the Wikidata knowledge base (KB) are sparse and incomplete. That is, many semantically related triples are not reflected in the KB. Therefore, treating such triples as negative instances (\textit{no\_relation}) will introduce false negative examples into the dataset. 
In the original DocRED production process, only the distantly supervised data is used to train the RE model, which may lead to low-quality prediction. 
Furthermore, the performance of the previously used RE model is significantly worse than the recent approaches based on pre-trained language models.
% The RE model did not use transformer-based pre-trained language model and its performance was significantly lower than the current SOTA. 
Therefore, the recommended relation triples from the RE model are likely not enough for covering the ground-truth relation triples for a given text.

By relying heavily on the relation triple candidates generated from the above two methods, the annotation of the previous DocRED dataset is incomplete.
While the recommend-revise scheme is the major source of the incompleteness of the original DocRED dataset \citep{yao2019docred}, a secondary source of incompleteness comes from logical inconsistency. 
There are many inverse relation pairs in DocRED. 
For example, if entity A is annotated as a \textit{sibling} of entity B, then entity B is also a \textit{sibling} of entity A. The lack of inverse relation also contributes to the incompleteness problem.
% \subsection{Problems of the DocRED dataset}
% \label{sec:problem-docred}

% In our preliminary investigations, we found that the DocRED dataset is flawed in following aspects.

% \noindent\textbf{Incomplete Annotation} As described in the previous section, the human annotation for relation triples was related to stage 1. distant supervision and stage 4. relation triple annotation. (\textcolor{red}{will double check the stage name, this is different and inconsistent with the previous section.}) Specifically, the annotators are asked to classify triples from distant supervision and predictions of neural RE models trained with the distantly supervised data. However, knowledge base that was used for distant supervision can be highly sparse and incomplete.




\subsection{The Impact of False Negatives}

To identify the difficulty of relation extraction, we conduct a preliminary analysis on two evaluation tasks: Relation Extraction (RE) and Positive Relation Classification (PRC).

\paragraph{Settings of Our Analysis}
Consider a text $T$ and a set of $n$ entities $\{e_1, ..., e_n\}$. $e_i$ and $e_j$ denote two different entities, and $R$ is a set of predefined relations, including \textit{no\_relation}. The objective of the RE task is to identify the relation type in $R$ for each entity pair $(e_i, e_j)$.  
% We also design a positive relation extraction setting to analyse the quality of the annotated triples that having relations.
Under the PRC setting, we do not use any entity pairs of \textit{no\_relation}, and the model is trained and evaluated with only entity pairs that have some pre-defined relation types.
Such a setting allows us to assess the difficulty of differentiating the predefined relation types.
%help to mitigate the potential issue of false negative.
We use the top-performing models for our preliminary experiments, and we report the scores on the development sets in these experiments. For the sentence-level task, we use the typed entity marker \citep{zhou2021improved} with RoBERTa-large~\citep{liu2019roberta} as our baseline. 
For the document-level task, we use KD-DocRE \citep{tan2022document} as the baseline. We use RoBERTa-large as the encoder for DocRED and XLM-R-base~\citep{conneau2020unsupervised} for HacRED.  
%\textcolor{red}{will include more details in the appendix, such as bert base or large.}

\paragraph{Datasets}
We compare the preliminary investigation results on two sentence-level RE datasets: TACRED \citep{zhang-etal-2017-position} and Re-TACRED~\cite{stoica2021re}, and two document-level RE datasets: DocRED \citep{yao2019docred}  and HacRED~\citep{cheng-etal-2021-hacred}. Table \ref{tab:data-stats} shows the statistics of the datasets.
Re-TACRED revised the TACRED dataset to reduce annotation errors.
% The TACRED dataset is a highly popular sentence-level RE benchmark with 42 relation types. \citet{stoica2021re} showed that the TACRED benchmark contains significant amount of annotation errors and provided a re-annotated version of TACRED (Re-TACRED). Compared to TACRED, Re-TACRED has a more refined label space with 40 relation types. 
Besides, we also create an incomplete Re-TACRED dataset, where 30\% of the positive labels are replaced with \textit{no\_relation} in the training, development, and test sets. 
This modification artificially creates false negative samples. This is to show the detrimental effect of the incompleteness problem on downstream tasks.
%due to false negative samples. 
DocRED and HacRED are document-level relation extraction datasets in English and Chinese, respectively.
% The DocRED dataset is a large-scale human-annotated document-level English RE dataset based on Wikipedia articles. It contains 96 relations from the Wikidata knowledge base. 
% The HacRED dataset is a Chinese document-level RE dataset that focused on 26 semantically hard relation types. 
For sentence-level relation extraction datasets, the negative ratio is typically lower than that of the document-level datasets, mainly because the complexity of relation extraction is quadratic in the number of entities. Therefore, document-level RE is more prone to the false negative problem.
%\textcolor{red}{will remove this once fix line 49.}
%\textcolor{red}{will verify the sentence-level data.} 
% For a given context $d$, the number of entity within the context is denoted as $m$, for the sentence level relation extraction, each example contains $m=2$ entities and 1 relation. Whereas for document-level relation extraction, one is asked to classify all possible entity pair permutations within one document, there are $m(m-1)$ classification decisions to be made and $m$ can be significantly larger than 2, for example, the DocRED benchmark has average entity number of $m=19.5$ and the HacRED has has average entity number of $m=10.8$. 
% For the positive relation classification task, given the context and entity pairs that having relation, the task is to determine the relation types for all the given entity pairs.
% The first task is positive relation extraction, where the context and entity boundaries are given and the task is to classify the relations for all the given entity pairs, whereas all entity pairs at least contain one type of relation. The second task is relation extraction, which adds a large amount of negative examples to the positive relation extraction task, since most entity pairs in real-world knowledge base do not have any relation. 
% In sentence-level relation extraction, negative examples typically consist of 80\% of the evaluation datasets, for instance, the sentence-level TACRED dataset \citep{zhang-etal-2017-position} has a negative ratio of 79.5\%. The negative ratio is significantly higher for document-level relation extraction datasets (Table.~\ref{tab:data-stats}), this is mainly because the complexity of relation extraction is quadratic to the number of entities $m$. 
% In this section, we show the preliminary investigation results for two sentence-level RE datasets: TACRED and Re-TACRED, and two document-level RE datasets: DocRED and HacRED. The TACRED dataset is a highly popular sentence-level RE benchmark with 42 relation types. \citet{stoica2021re} showed that the TACRED benchmark contains significant amount of annotation errors and provided a re-annotated version of TACRED (Re-TACRED). Compared to TACRED, Re-TACRED has a more refined label space with 40 relation types. Besides, we also experimented on a artificially corrupted Re-TACRED dataset, where 30\% of the positive labels are changed to `\textit{no\_relation}' in the train, development and test set. Intuitively, the modified labels are artificially created false negative examples. This is to show the detrimental effect from the false negative examples. The DocRED dataset is a large-scale human-annotated document-level English RE dataset based on Wikipedia articles. It contains 96 relations from the Wikidata knowledge base. The HacRED dataset is a Chinese document-level RE dataset that focused on 26 semantically hard relation types. We use the state-of-the-art models for the preliminary experiments. For the sentence-level experiments, we use the \textit{typed entity marker} \citep{zhou2021improved} as our baseline model. For the document-level experiments, we use the ATLOP model \citep{zhou2021document} as our baseline model.  

\begin{table}[t!]
\centering
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lccc} 
\toprule
 \textbf{Dataset}         & P     & R   & F1    \\ 
\midrule
\multicolumn{2}{l}{\textbf{Sentence-level}} \\ 
TACRED    & 93.38 & 93.38 & 93.38  \\
Re-TACRED & 96.83 & 96.83  & 96.83  \\
Incomplete Re-TACRED & 96.53 & 96.53  & 96.53 \\ 
\midrule
\multicolumn{2}{l}{\textbf{Document-level}}  \\ 
DocRED    & 93.33 & 90.28 & 91.78  \\
HacRED    & 95.18 & 94.95 & 95.07  \\
\bottomrule
\end{tabular}
}
% \vspace{-0.15cm}
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{-10pt}
\caption{Preliminary experimental results of PRC.}
\label{tab:pos-rel}
\end{table}

% \textcolor{red}{ADD: justify the reasons why we compare different models on different datasets.}

\subsubsection{Preliminary Results of Positive Relation Classification}
\label{sec:prc}
By assuming that there is a relation between the entity pairs, the positive relation classification (PRC) task shows the difficulty of differentiating the relation types. 
Note that document-level PRC is a multi-label classification problem. Hence, precision and recall are not necessarily the same.   
% The positive relation classification task shows the difficulty of classifying the relation labels, which presumes there is a relation between the entity pairs. 
From Table~\ref{tab:pos-rel}, we can see that all the models perform well. 
The performance of sentence-level RE and document-level RE are comparable, even though document-level RE has a significantly longer context and requires cross-sentence reasoning. 
This shows that the difficulty of positive relation classification is not severely affected by sentence boundary or context length. 
Another finding from Table~\ref{tab:pos-rel} is that the revised version of TACRED has marginally higher performance than the original version. This is expected as the revised version receives an extra round of human annotation. 
The performance on Incomplete Re-TACRED is only marginally worse than Re-TACRED, which shows that positive relation classification can achieve a comparatively high performance despite the reduction of training instances. 
Besides, it is worth noting that the performance on HacRED is higher than the performance on DocRED, even though HacRED claims that it is a semantically harder dataset. 
Although the baselines are not exactly the same, we can still infer that the difficulty level of classifying the positive relation types on sentence-level and document-level datasets is not significantly different.
% From Table~\ref{tab:pos-rel}, we can see that the existing large neural models are able to perform well on classifying the relation types on both sentence-level and document-level.


\begin{table}[t!]
\centering
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lccc} 
\toprule
\textbf{Dataset} & P     & R    & F1     \\ 
\midrule
\multicolumn{2}{l}{\textbf{Sentence-level}}  \\ 
TACRED    & 75.70 & 	73.40 & 74.50  \\
Re-TACRED & 90.60	& 91.30   & 90.90 \\
Incomplete Re-TACRED & 65.61 & 71.71  & 68.52 
  \\ 
\midrule
\multicolumn{2}{l}{\textbf{Document-level}} \\
DocRED    & 64.62 & 63.53 & 64.07  \\
HacRED    & 78.45 & 77.93 & 78.19  \\
\bottomrule
\end{tabular}
}
% \vspace{-0.15cm}
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{-10pt}
\caption{Preliminary experimental results of RE.}
\label{tab:rel-extraction}
\end{table}


\subsubsection{{Preliminary Results of Relation Extraction}}

% The experiment results of relation extraction is shown in Table~\ref{tab:rel-extraction}. 
Compared to the setting of positive relation classification, the standard relation extraction task includes all the negative \textit{no\_relation} samples during training.
We compare the performance of the previous best approaches on the sentence-level and document-level RE datasets in Table~\ref{tab:rel-extraction}.
We observe that the performance on the standard RE task is lower than that on the PRC task. For a specific dataset, the performance on PRC is the upper bound of RE performance, since the evaluation of PRC ignores \textit{no\_relation}.
%This is because the standard RE task requires determining if there exists a relation for a given triple.
However, the performance between relation extraction and positive relation classification should not have a large gap, as the positive samples should be semantically different from the negative samples for a well-annotated dataset.
% if the annotated negative examples are semantically different from the positive examples. 
For the sentence-level dataset, we can see that the performance on the revised version of TACRED (Re-TACRED) is significantly higher than that of the original TACRED dataset.
The performance difference between the positive relation classification and relation extraction is 18.88 (93.38 vs. 74.50) F1 score for TACRED, whereas the gap is only 5.93 (96.83 vs. 90.90) F1 score for Re-TACRED. For the incomplete Re-TACRED, this gap becomes 28.01 (96.53 vs. 68.52). Moreover, from the comparison of Re-TACRED and incomplete Re-TACRED, we can see that the performance of PRC only dropped  by 0.3 (96.83 vs. 96.53), whereas the performance of RE dropped by 22.38 (90.90 vs. 68.52). This shows that the incompleteness problem greatly decreases RE performance even if the positive instances are precisely labeled, whereas the performance of PRC is not significantly affected by the incompleteness problem. 
% Should emphasize this part, since incompleteness can highly affect the performance of RE while having minimal effect on PRC. 
% This observation shows that the Re-TACRED dataset significantly corrects the false negative examples throughout the training and evaluation sets of TACRED. \textcolor{red}{too strong}
For the document-level datasets, we observe large gaps between  positive relation classification and relation extraction, 27.71 (91.78 vs. 64.07) F1 for DocRED and 16.88 (95.07 vs. 78.19) for HacRED, respectively.
Compared to the 5.93 F1 gap on the Re-TACRED dataset, the gaps of PRC and RE on the document-level datasets are significantly larger. These observations indicate that there may exist a substantial number of false negative examples throughout the training, development, and test sets of these datasets.  
Therefore, it is necessary to re-check the quality of the document-level relation extraction datasets.
% We observe that the performance of sentence-level RE and document-level RE are no longer comparable. 
% With all the negative examples, the performance of RE models are expected to drop, since the evaluation protocol of RE task neglects \textit{"no\_relation"} labels. 
% If the negative examples are labeled correctly, the performance for relation extraction and positive relation extraction should be comparable.
% We can see that the performance for the revised version of TACRED (Re-TACRED) performs significantly higher than the original TACRED dataset and the performance gap is 16.4 F1 score, whereas their performance gap is only 3.7 F1 score in the positive relation classification task. 
% This observation shows that the re-annotation effort of Re-TACRED is mainly correcting the false negative examples throughout the training and evaluation sets of TACRED. Moreover, from the comparison of Re-TACRED and its incomplete counterpart, we can see that false negative examples can have highly poisonous effect on RE performance even if the positive instances are precisely labeled.




==> EMNLP_2022/sections/3_methodology.tex <==
\section{Revising DocRED with an Iterative Approach}
\label{sec:revision}
In this section, we describe our iterative human-in-the-loop approach to revise DocRED.
The goal is to add the previously unrecognized relation triples to the DocRED dataset. 
Our iterative approach consists of three steps in each iteration: 
(1) Training scorer models;
(2) Scoring all possible triples; and
(3) Human verification.
The following sections provide the details of each step.

\begin{table}[ht]
\centering
\begin{tabular}{llll} 
\toprule
Split 0~ & Split 1 & Split 2 & Split 3  \\ 
\midrule
1,000  & 1,000 & 1,000 & 1,053  \\
\bottomrule
\end{tabular}
\caption{Dataset statistics of each split. Split 0 is the original DocRED development set.}
\label{tab:data-split}
\end{table}  

\subsection{Our Iterative Approach}
\label{sec:iterative}
\paragraph{Step 1 - Training Scorer Models}
\label{sec:step1}
Even though the annotation of the previous DocRED is incomplete, we can still train neural models on such data.
We adopt three top-performing models on the current DocRED leaderboard: KD-DocRE~\cite{tan2022document}, DocuNET~\citep{zhang2021document}, and ATLOP~\citep{zhou2021document}. 
To obtain relation triple candidates for all 4,053 documents, we split the original DocRED into 4 different splits (Table~\ref{tab:data-split}), with the first split as the original DocRED development set. This is to ensure that the number of training samples is comparable to the original DocRED when any three of the splits are used for training our scorer models, and the remaining split is used for prediction. Following the training paradigm of \citet{tan2022document}, we first pre-train each model with the distantly supervised data in DocRED. Then, the pre-trained model is further trained on any three splits of DocRED,
and we then use the trained model to make predictions on the remaining split. Therefore, it requires four rounds of training and inference so that we can get the predictions for all the four splits.

% \footnote{We used all four splits for round one and one split for round two.}. 
%We then train each model in a cross-validation manner, i.e., when three parts are used for training, the remaining one part is used for evaluation.
%\footnote{Note the differences of round 1 and round2. \textcolor{red}{revise later.}}
%Furthermore, we apply methods in positive-unlabeled learning~(PU learning) to improve the recall of the models' output. 
%\textcolor{red}{ add more details for PU?}

%Need for Unrecognized
\paragraph{Step 2 - Scoring the Triples}
\label{sec:cand-generation}
In this step, we aim to generate a large number of relation triple candidates, so that they could cover the missing annotations in the previous DocRED.
With the trained scorer models, we can predict the scores for all the enumerated relation triples.
To control the number of relation triple candidates for the next step, we define a threshold score to remove the less confident predictions. Specifically, we set the dynamic threshold to 0.9 of the models for the Adaptive Threshold class \citep{zhou2021document} for all trained models. 
The predicted relation triples from all the models are then merged together.
Due to the different characteristics of these models, we could generate a large and diverse pool of relation triple candidates for the next step. By default, the original positive triples from DocRED are treated as correct and are not  re-annotated.


\paragraph{Step 3 - Human Verification}
After the relation triple candidates are generated from the previous step, each triple candidate will be annotated by humans. The human annotators are asked to read the document and check whether the triples can be inferred from the document. %Unlike the annotation process of the original DocRED, we did not ask the annotators to explicitly label the supporting evidence of their judgment. This is mainly because the evidence annotations have a marginal effect on RE and they are hard to obtain during inference time. 
Each triple will be annotated by two annotators, and a third annotator will resolve the conflicting annotations. 

%The above three steps form one round of our iterative approach.

% \textcolor{red}{repeated sents}

% \subsection{Supplementation with Logical rules}
% \label{sec:logic}
% After human annotation, we also supplement relation triples by manually defining logic rules. In this way, we are able to resolve the probel of logical inconsistencies (described in Section \ref{sec:problem-docred}) in the DocRED dataset. These rules mainly consist of inverse relations and co-occurring relations. On average, we supplemented  6.4 triples for each  document.
% % 6.2 triples for each training document and 6.7 for each evaluation document.

\begin{table}[t]
\centering

\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc} 
\toprule
                      \multirow{2}{*}{\textbf{Dataset}}    & \multicolumn{3}{c}{\textbf{Re-DocRED}}        & \multicolumn{2}{c}{\textbf{DocRED}}  \\
                          \cmidrule(lr){2-4} \cmidrule(lr){5-6}
                          & \textbf{Train} & \textbf{Dev} & \textbf{Test} & \textbf{Train} & \textbf{Dev}        \\ 
\midrule
\textbf{\# Documents}      & 3,053          & 500          & 500           & 3,053          & 1,000               \\
\textbf{Avg. \# Entities}  & 19.4           & 19.4         & 19.6          & 19.5           & 19.6                \\
\textbf{Avg. \# Triples}   & 28.1           & 34.6           & 34.9          & 12.5           & 12.3                \\
\textbf{Avg. \# Sentences} & 7.9            & 8.2          & 7.9           & 7.9            & 8.1                 \\
\bottomrule
\end{tabular}}
% \vspace{-0.15cm}
% \setlength{\belowcaptionskip}{-8pt}
\caption{Statistics of Re-DocRED and DocRED. }
\label{tab:data-stats-doc}
\end{table}



\begin{table*}
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccccc} 
\toprule
\multirow{3}{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{DocRED}} & \multicolumn{4}{c}{\textbf{Re-DocRED}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Test Differences}}}   \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
\multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{Dev}}                              & \multicolumn{2}{c}{\textbf{Test}}                             & \multicolumn{2}{c}{\textbf{Dev}}                              & \multicolumn{2}{c}{\textbf{Test}}                             &   \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
& \multicolumn{1}{c}{Ign\_F1} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Ign\_F1} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Ign\_F1} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Ign\_F1} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{$\Delta$Ign\_F1} & \multicolumn{1}{c}{$\Delta$F1}  \\ 
\midrule
JEREX                & 57.07	                       & 58.97	                 & 57.14	                       & 59.01                  &  71.59	                 & 72.68                & 	71.45                  & 72.57                     & $+$14.31	                             & $+$13.56                        \\
ATLOP                & 61.21	                       & 63.07	                 & 61.44                      & 	63.20                    & 76.79                     & 	77.46                  & 	76.82	                       & 77.56                  & $+$15.38	                            & $+$14.36                         \\
DocuNET              & 61.62	                     & 63.53	                  & 61.80	                      & 63.64                  & 77.49                     & 	78.14	                   & 77.26                       & 	77.87               & $+$15.46		                             & $+$14.23                           \\
KD-DocRE                & 62.08	                      & 64.07	                   & 62.21	                       & 64.07                   & 77.85                            & 	78.51       & 77.60               & 	78.28                           & $+$15.39	                             & $+$14.21 
  \\ 
\midrule
\multicolumn{6}{l}{\textbf{+ Pre-trained with distantly supervised data}}  \\JEREX                & 60.39	                       & 62.24	                 & 60.29	                        & 62.15                  & 73.34	                      &74.77	                   & 73.48                       & 	74.79                  & $+$13.19	                             & $+$12.64                         \\
ATLOP                & 63.68	                       & 65.61	                & 63.63	                        & 65.51                  & 78.32	  		         & 79.26	                  & 78.52	                    & 79.46	                   & $+$14.89	                           & $+$13.95                          \\
DocuNET              & 63.22                     & 	65.25	                   & 63.23                      & 	65.26                   & 78.20	                       & 78.90	                 & 78.28	                       & 78.99	                  & $+$15.06		                            & $+$13.73  \\
KD-DocRE                & 65.11                       & 	67.04	                  & 65.21                     & 	67.09                    & 79.79	                         & 	80.56		               & 80.32               & 		81.04	                 & $+$15.11			                           & $+$13.95                         \\
\bottomrule
\end{tabular}
}
% \vspace{-0.15cm}
% \setlength{\abovecaptionskip}{.1pt}
% \setlength{\belowcaptionskip}{-8pt}
\caption{Experimental results using the original DocRED and our Re-DocRED. The reported numbers are average scores over 3 runs. The reported DocRED results use the same splits of development and test sets as Re-DocRED.}
\label{tab:revised-exp-no-ds}
\end{table*}





\subsection{Our Revised Re-DocRED}
\label{sec:re-docred-stats}
The above three steps form one round of our iterative approach. We conducted two rounds of annotation in total. For the first round, we annotated 4,053 documents that include all training and evaluation documents. On average, we recommended 11.9 triples for each document and 9.4 triples were accepted, with an acceptance rate of 79.0\%. The Fleiss Kappa~\citep{fleiss1971measuring} coefficient for round 1 annotation is 0.73, which is considered as substantial agreement. To further improve the recall on the evaluation dataset, we conducted a second round of annotation for the 1,000 evaluation documents. We used the annotated 3,053 training samples from round 1 for round 2 training. 
In this round, 14.1 triples were recommended and only 6.0 triples were accepted, with an acceptance rate of only 42.6\%. The Fleiss Kappa coefficient for round 2 annotation is 0.66.
After human annotation, we also add relation triples by manually defining logical rules. In this way, we are able to resolve the problem of logical inconsistency (described in Section \ref{sec:problem-docred}) in the DocRED dataset. These rules mainly consist of inverse relations and co-occurring relations. See Appendix \ref{app:logic-detail} for more details.
%On average, we added 6.4 triples for each  document. 
%Since our main goal is to address the false negative problem in the DocRED dataset, we keep all the existing annotated triples in the original DocRED dataset.
Overall, our training documents contain 28.1 triples on average, with 9.4 triples added from human annotation and 6.2 triples from logical rules. Our evaluation documents contain 34.7 triples on average, with 15.7 triples added from human annotation and 6.7 triples from logical rules. We divide the 1,000 evaluation documents into 500 development and 500 test documents. The average number of triples of the evaluation documents is higher than that of the training documents. This indicates that the evaluation data has more complete annotation compared to the training data. The detailed statistics of the Re-DocRED dataset are shown in Table~\ref{tab:data-stats-doc}. The average number of triples per document is significantly higher for Re-DocRED compared to the original DocRED. There are 12.3 triples per document in the DocRED dev set and 34.7 triples per document in the dev and test sets of Re-DocRED. This shows that approximately 64.6\% of all triples are missing in the original DocRED dataset.



%\textcolor{red}{will modify this when data is updated.}
%\textcolor{red}{will include the acceptance rate and the differences between train and dev test.} 
%Will clarify this part with round 2 annotations, now is the same percentage





==> EMNLP_2022/sections/4_experiments.tex <==
 \section{Experiments}













\subsection{Comparison on Relation Extraction}
\label{sec:experiment-compare}
To compare the previous DocRED and our Re-DocRED, we evaluate 4 different approaches on the two datasets.
Apart from the three models that are used during our annotation process (Section~\ref{sec:step1}), we also compare the performance with an additional approach, JEREX \cite{eberts2021end}. This approach is not included in our data production process and we use it as an independent model to compare DocRED and Re-DocRED.
% We compared all the models under two different settings: 
% the first is \textbf{\textit{Silver Label}} setting, which is to train with the human-annotated portion only, we denote this setting as ``Silver Label'' because even though the Re-DocRED dataset have supplemented large amounts of triples to the original DocRED, there may still be some missing annotations in the training set of Re-DocRED, hence the training set is not ``gold label''. 
% The second setting that we used is \textbf{\textit{DS + Silver Label}} setting, where both distantly supervised data and human-annotated data are used for training.
Table~\ref{tab:revised-exp-no-ds} shows the experimental results, and the reported metrics are micro-averaged F1 scores and Ign\_F1 scores. The latter refers to the F1 score that ignores the triples appearing in the training set.
According to the statistics in Table \ref{tab:data-stats}, even though our revised Re-DocRED dataset contains many more relation triples, we observe that all the baseline models demonstrate significant performance improvement on both development and test sets. 
Compared to DocRED, the performance of the baseline models on Re-DocRED increased by more than 12 F1 points. 
When these models are pre-trained with distantly supervised data\footnote{{There are 101K distantly supervised documents in the original DocRED dataset.}}, we observe consistent performance improvement on Re-DocRED. We also further analyze the error cases of the SOTA model in Appendix~\ref{sec:model-mistakes}.

%\textcolor{red}{need a new data statistics table to show the difference of the two versions, in terms of train dev?}
%\textcolor{red}{explain the reason why more significant?}



\begin{table}[t]
\centering
% \vspace{0.1cm}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{llccc} 
\toprule
\textbf{Training}     & \textbf{Test}      & P     & R    & F1     \\ 
\midrule
DocRED    & DocRED    & 93.33 & 90.28 & 91.78  \\
Re-DocRED & Re-DocRED & 95.03 & 90.55 & 92.74  \\
\bottomrule
\end{tabular}}
% \vspace{-0.1cm}
% \setlength{\abovecaptionskip}{3pt}
% \setlength{\belowcaptionskip}{-6pt}
\caption{Positive relation classification performance with the original DocRED and our revised Re-DocRED (using KD-DocRE).}
\label{tab:pos-rc-rev}
\end{table}


\begin{table*}[ht]
\centering
\resizebox{0.8\textwidth}{!}{\begin{threeparttable}
\begin{tabular}{lcccccccc} 
\toprule
\multirow{2}{*}{\textbf{Model}}& \multicolumn{2}{c}{\textbf{Dev}} &\multicolumn{6}{c}{\textbf{Test}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-9}
& \textbf{Ign\_F1} & \textbf{F1}    & \textbf{Ign\_F1} & \textbf{F1}    & \textbf{Freq. F1} & \textbf{LT F1} & \textbf{Intra F1} & \textbf{Inter F1}  \\ 

\midrule
JEREX   & 71.59                            & 	72.68	           & 71.45                 & 	72.57               & 77.09		              & 66.31              & 		76.10	           & 	69.88                   \\
ATLOP   & 76.79                             & 	77.46	           & 76.82                  & 	77.56               & 80.78	              & 72.29               & 	80.11	           & 74.92                  \\
DocuNET & 77.49                 & 	78.14	           & 77.26	                           & 77.87                  & 81.25                & 73.32                & 	79.89	                & 76.58                 \\
KD-DocRE   & 77.85	                     & 78.51	         & 77.60                             &	78.28	                 & 80.85	               & 74.31	              & 79.52	                & 77.18   \\
\midrule
\multicolumn{6}{l}{\textbf{+ Pre-trained with distantly supervised data}}  \\
JEREX   & 73.34		                             &74.77		            & 73.48	               & 	74.79        & 	78.67	 	                      & 68.62		              & 76.90		               & 72.65                 \\
ATLOP   & 78.32	                             &79.26	            & 78.52                & 	79.46          & 	82.23	                      &75.17	              & 80.39	               & 78.44                  \\
DocuNET & 78.20	                              & 78.90	                & 78.28               & 	78.99	                 & 82.08                & 	74.19                &	80.46	              & 77.72                 \\
KD-DocRE   & 79.79                      & 	80.56                      & 	80.32	                & 81.04	                & 83.17	               & 79.31	                 & 82.01	                & 79.87      \\
\bottomrule
\end{tabular}
\end{threeparttable}
}
% \vspace{-0.15cm}
% \setlength{\abovecaptionskip}{3pt}
% \setlength{\belowcaptionskip}{-10pt}
\caption{Performance comparison under different metrics on the Re-DocRED dataset. }
\label{tab:benchmark}
\end{table*}



\subsection{Comparison on Positive Relation Classification}
Following the experimental setting in Section \ref{sec:prc},  
we compare the positive relation classification performance between the original DocRED and our Re-DocRED with KD-DocRE~\citep{tan2022document} in Table~\ref{tab:pos-rc-rev}. 
The performance on Re-DocRED is slightly better than that on the original DocRED. 
This indicates that our added triples are of comparable quality to the original DocRED data.



% \begin{table*}[ht]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcc|cccccc} 
% \hline
%                      & \multicolumn{2}{c}{\textbf{Dev}}     & \multicolumn{6}{c}{\textbf{Test}}                                            \\
% \textit{Distantly Supervised} & \textbf{Ign\_F1}             & \textbf{F1}    & \textbf{Ign\_F1} & \textbf{F1}    & \textbf{Freq. F1} & \textbf{LT F1} & \textbf{Intra F1} & \textbf{Inter F1}  \\ 
% \hline
% ATLOP                & 59.44               & 60.6  & 59.51   & 60.88 & 67.45       & 52.51        & 64.22    & 57.66     \\
% DocuNET              & 56.01               & 57.65 & 55.96   & 57.58 & 63.99       & 49.93        & 59.29    & 56.02     \\
% KD-DocRE                & 63.97               & 64.88 & 63.87   & 64.79 & 71.73       & 57.27        & 67.36    & 62.49     \\ 
% \hline
% \multicolumn{2}{l}{\textit{Paritially Annotated}}   &       &         &       &             &              &          &           \\ 
% \hline
% ATLOP                & 58.71               & 60.85 & 58.58   & 60.41 & 65.61       & 56.36        & 66.58    & 56.17     \\
% DocuNET              & 60.55               & 61.15 & 60.61   & 61.25 & 65.01       & 56.25        & 66.24    & 55.97     \\
% KD-DocRE                & 61.94               & 62.89 & 61.86   & 62.77 & 67.93       & 56.7         & 67.87    & 57.72     \\ 
% \hline
% \multicolumn{2}{l}{\textit{Silver Labeled}}         &       &         &       &             &              &          &           \\ 
% \hline
% ATLOP                & 75.55               & 76.77 & 75.43   & 76.64 & 80.36       & 71.16        & 78.77    & 74.17     \\
% DocuNET              & 75.98               & 77.19 & 75.94   & 77.17 & 81.09       & 72.16        & 79.81    & 74.80      \\
% KD-DocRE                & 76.54               & 77.94 & 76.41   & 77.65 & 81.63       & 74.15        & 79.88    & 76.37     \\ 
% \hline
% \multicolumn{2}{l}{\textit{DS + Silver Labeled}}   &       &         &       &             &              &          &           \\ 
% \hline
% ATLOP                & 79.11               & 80.42 & 79.27   & 80.67 & 83.55       & 76.67        & 82.88    & 78.53     \\
% DocuNET              & 78.67               & 79.95 & 78.70    & 80.04 & 83.64       & 75.25        & 81.61    & 78.52     \\
% KD-DocRE                & 81.54               & 82.58 & 81.44   & 82.54 & 85.45       & 78.78        & 84.13    & 81.01     \\
% \hline
% \end{tabular}
% }

% \caption{Benchmark settings for the document-level RE task. \textcolor{red}{change to analysis on dev sets if have time.}}
% \label{tab:benchmark}
% \end{table*}
%\textcolor{red}{change the name of FULL to silver, as we cannot have a gold annotation.}
% As shown in Table~\ref{tab:revised-exp-no-ds}, the performances of neural models on our Re-DocRED dataset have improved significantly. To better analyze the performance breakdown of the document-level RE task, 
% we propose additional two benchmark settings:
% 1). \textbf{\textit{Distantly Supervised}} setting, 2). \textbf{\textit{Partially Annotated}} setting,
% % we propose the following four benchmark settings: 
% % 1). \textbf{Distantly Supervised Setting}, 2). \textbf{Partially Annotated Setting}, 3). \textbf{Silver Labeled Setting} and 4). \textbf{DS + Silver Labeled Setting}. 

% Besides the \textbf{\textit{Silver Labeled}} setting and \textbf{\textit{DS + Silver Labeled}} setting shown in section~\ref{sec:experiment-compare}, the  \textbf{\textit{Distantly Supervised}} setting and the \textbf{\textit{Partially Annotated}} setting are two more practical settings for document-level RE. 
% With our high quality evaluation sets, we realize that it is not always necessary to have such an effort-intensive annotation for the training set. As such, the \textbf{\textit{Distantly Supervised}} setting requires models to learn from the noisy distantly supervised data, where both false positive and false negative labels are prevalent, and the trained models will be evaluated on our clean evaluation sets. 
% Regarding the \textbf{\textit{Partially Annotated}} setting, the previous incompletely annotated training set of DocRED is provided during training, but the evaluation is conducted on our high-quality evaluation sets. 
% % On the other hand, the \textbf{Partially Annotated Setting} asks one to train with the original DocRED training set and evaluation is conducted on our high-quality evaluation sets. 
% This scenario presumes that there is a small amount of precise human-annotated data (no false positives), whereas the annotation is incomplete (with many false negatives).


%As mentioned in Section \ref{sec:revision}, both the development and test sets are annotated 4 times with an additional round of quality checking to address the annotation inconsistency. 

% It is worthwhile to explore the methods of relying on the available distant supervision data or the partially annotated data to achieve comparable performance as using the silver labeled data. Besides different benchmark settings, 









%\subsection{Partially Annotated Setting}

% \noindent\textbf{Fully Annotated Setting.}

% \noindent\textbf{portion of Fully Annotated Setting.}

% \noindent\textbf{DS + Fully Annotated Setting.}

 %\textcolor{red}{cross compare the PRC with different combination of postive data.}



==> EMNLP_2022/sections/5_analysis.tex <==
\subsection{More Analysis}
\label{sec:analysis}


\paragraph{Additional Evaluation Metrics} As mentioned in Section \ref{sec:preliminaries}, document-level relation extraction is a challenging task. Hence, it is necessary to have various performance evaluation metrics so as to conduct a comprehensive evaluation.
%define
On top of the standard F1 and Ign\_F1 evaluation metrics, we use four additional metrics to assess the models. 
(1) \textbf{Freq. F1}~\citep{tan2022document}, which only considers the 10 most common relation types in the training set of Re-DocRED, where these frequent relation types account for around 60\% of the relation triples. 
(2) \textbf{LT F1}, which only considers the long-tail (the remaining 86) relation types. 
(3) \textbf{Intra F1}~\citep{nan-etal-2020-reasoning}, which evaluates on relation triples that appear in the same sentence. 
(4) \textbf{Inter F1}, which evaluates on cross-sentence relation triples. 

We show the comprehensive evaluation results in Table~\ref{tab:benchmark}. We observe that there exists a relatively large gap between the \textbf{Freq. F1} and \textbf{LT F1} metrics, and the difference is around 6 to 10 F1 points. Such behavior shows that the frequent relation types are easier to be recognized compared to the long-tail relation types.
Furthermore, we also find that the performance on triples that appear in the same sentence (\textbf{Intra F1}) is better than that on the cross-sentence relation triples (\textbf{Inter F1}), by around 2 to 6 F1 points. This is because it is harder to encode long-distance interactions.
%Therefore, a promising future direction is to match the performance on the long-tail relation types to the frequent types, and also improve the model's representation capability to capture long-distance interactions so as to reduce the differences between the inter-sentence and intra-sentence relation triples.
Therefore, future research can work on matching the performance of the long-tail relation types to the frequent types and also improve the model's representation capability to capture inter-sentence interactions.



%\noindent\textbf{Effects of Distant Supervision Pre-training} To further analyze the effects of distant supervision pre-training, we examine the performance of the KD-DocRE model with and without the pre-training step, and Table~\ref{p-r-by-class} shows the results.Under both settings, the recall of the long-tail classes is significantly lower than their corresponding precision. \bing{the previous sentence is also true for Freq.?}Moreover, by comparing the performance of long-tail classes, we observe that pre-training with distantly supervised data improves the precision of the long-tail classes. We show additional error analysis and case studies in Appendix~\ref{sec:model-mistakes}.
%\bing{This whole paragraph needs further thought.}

%\subsection{Effects of Distant Supervision Pre-training}
% \noindent\textbf{Analysis of P and R} \colorB{
% We also present the precision and recall scores of the KD-DocRE in Table~\ref{tab:negative-sampling}. To further analyze the performance breakdown of DocRE, we examine the performance of the KD-DocRE model, and Table~\ref{p-r-by-class} shows the results. 
%The default setting of existing SOTA models,  We elaborate this method in the next paragraph.} \bing{Table 8 has Freq. and LT, but they are not mentioned at all in the text. Also the result here cannot be compared with Table 9. }
%\bing{the previous sentence is also true for Freq.?}
%Moreover, by comparing the performance of long-tail classes, we observe that pre-training with distantly supervised data improves the precision of the long-tail classes. We show additional error analysis and case studies in Appendix~\ref{sec:model-mistakes}.
%\bing{This whole paragraph needs further thought.}


% From Table~\ref{tab:benchmark}, it can be seen that the absolute performance of document-level RE on F1 score has been significantly improved. 
\begin{table}[t]
\centering
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lcccc} 
\toprule
\textbf{Training}     & \textbf{Negative Sample}      & P     & R    & F1     \\ 
\midrule
DocRED    & All  &  92.08 & 32.07 & 47.57 \\
Re-DocRED & All & 89.76 & 69.40  & 78.28  \\
\midrule
DocRED    & Partial (10\%)    & 77.96 & 51.97  & 62.37\\
Re-DocRED & Partial (70\%)  & 83.58 & 75.06 & 79.09  \\
\bottomrule
\end{tabular}}
% \vspace{-0.15cm}
% \setlength{\abovecaptionskip}{3pt}
% \setlength{\belowcaptionskip}{-2pt}
\caption{Experimental results when using different numbers of negative samples. }
\label{tab:negative-sampling}
\end{table}


\paragraph{Training with DocRED vs. Re-DocRED}
We compare the performance of the KD-DocRE model when it is trained on the training sets of DocRED and Re-DocRED, and the results are shown in the upper section of Table \ref{tab:negative-sampling}. 
Note that for reliability, the evaluations are conducted on the development and test sets of Re-DocRED.
Under the default setting (using all the positive and negative samples during training), the model trained with the Re-DocRED training data achieves a comparable precision score as DocRED (89.76 vs. 92.08). 
However, the recall score of the model trained with Re-DocRED is much better than DocRED (69.40 vs. 32.07).
This demonstrates the severe incompleteness of the previous DocRED's annotation, and models trained with such data fail to capture many triples.
After adding back the missed samples, Re-DocRED's training set is more complete and thus the trained model tends to extract more valid triples.
Figure~\ref{fig:example-doc-pred} shows an example document with predictions of models trained on the two training sets. 
We can see that the model trained with Re-DocRED indeed outputs more correct triples.
%which is probably because the added back triples are mostly the same type of difficult ones.
On the other hand, for Re-DocRED, the recall score is still lower than the corresponding precision score. One possible reason is that the evaluation sets of Re-DocRED received two rounds of annotation while the training set only received one round. Therefore, the annotation of the evaluation sets of Re-DocRED is more complete compared to the training set.

To further compare the annotation quality, we conduct experiments to  randomly sample a subset of the negative samples instead of using all of them. This training strategy is known as negative sampling, and it is shown to be effective in resolving the false negative problem \citep{li2021empirical} during training for named entity recognition.
The experimental results on negative sampling are given in the lower section of Table~\ref{tab:negative-sampling}. 
When random down-sampling on negative entity pairs is adopted, the experimental results are improved, due to significantly improved recall.
We also observe that the improvement is more significant on DocRED. 
This demonstrates that the incompleteness problem of our revised training data is significantly alleviated. 
The sampling rate is a hyper-parameter obtained by grid search, and the details of negative sampling are described in Appendix~\ref{app:neg-sample-detail}.
% Our empirical observation showed that simple negative sampling could balance the precision and recall and improve the F1 score.


% \noindent\textbf{Negative Sampling}
% Since annotating document-level RE examples is expensive, finding methods to learn from incomplete annotation is important. The default setting of all current SOTA models (\citealp{tan2022document}; \citealp{zhang2021document}; \citealp{zhou2021document}) is using all possible negative entity pairs during training. Our empirical observation showed that simple negative sampling could balance the precision and recall and improve the F1 score. This is also observed in the unlabeled named entity recognition problem \citep{li2021empirical}. We show the experiment results on negative sampling in Table~\ref{tab:negative-sampling}. We can see that random down-sampling on negative entity pairs can improve the performance on the Re-DocRED's test set. The performance improvement is more significant when the original version of DocRED is used for training. This also showed that the incompleteness problem of our revised training data is significantly alleviated. The sampling rate is a hyper-parameter and obtained by grid search, the details of negative sampling are described in Appendix~\ref{app:neg-sample-detail}.





\begin{figure}[!t]
\centering
\small
\begin{tabular}{|p{0.92\columnwidth}|}
\hline
\vspace{-.1cm}
\textbf{Ross Patterson Alger} ( \textbf{August 20 , 1920} – \textbf{January 16 , 1992} ) was a politician in the \textbf{Canadian} province of \textbf{Alberta} , who served as mayor of \textbf{Calgary} from 1977 to 1980 . Born in \textbf{Prelate} , \textbf{Saskatchewan} , he moved to \textbf{Alberta} with his family in 1930s . He received a bachelor of commerce degree from the \textbf{University of Alberta} in \textbf{1942} . \colorbox{LightYellow}{\underline{He served with the}} \textbf{Royal Canadian Air Force} during \textbf{World War II} . After the war , \colorbox{LightYellow}{\underline{he received an MBA from the}} \textbf{University of Toronto}...  \\
\vspace{0.05cm}
\textbf{Subject Entity}: \textbf{Ross Patterson Alger}\\
\textcolor{orange}{\textbf{DocRED}}: (\textit{place of birth},  \textbf{Prelate}), (\textit{date of birth}, \textbf{August 20 , 1920}), (\textit{educated at}, \textbf{University of Alberta})...  \\
\vspace{0.05cm}
\textcolor{skyblue}{\textbf{Re-DocRED}}: (\textit{place of birth}, \textbf{Prelate}), (\textit{date of birth}, \textbf{August 20 , 1920}), (\textit{educated at}, \textbf{University of Alberta}), \color{darkgreen}{(\textit{educated at}, \textbf{University of Toronto})}, \color{darkgreen}{(\textit{military branch}, \textbf{Royal Canadian Air Force})}... 
\vspace{.1cm}\\
\hline
\end{tabular}
% \setlength{\abovecaptionskip}{0pt}
% \vspace{-0.15cm}
% \setlength{\belowcaptionskip}{-12pt}
\caption{Sample predictions of the model when it is trained on DocRED and Re-DocRED training sets, and the subject entity of the selected triples is ``Ross Patterson Alger''. 
The \colorbox{LightYellow}{\underline{highlighted evidence}} verifies that the model trained on Re-DocRED has captured more correct inter-sentence triples (\textcolor{darkgreen}{colored in green}) \color{black}{than DocRED}.}
\label{fig:example-doc-pred}
\end{figure}

%\bing{for DocRED, 10\% is not the boundary condition.}

==> EMNLP_2022/sections/6_related.tex <==

\section{Related Work}

\paragraph{Relation Extraction}
% Relation extraction (RE) is an important task in information extraction and knowledge graph completion. 
There is a series of relation extraction datasets built over the past decades, and they have significantly advanced research on RE. 
ACE 2005 \citep{walker2006ace} and SemEval 2010 Task 8~\citep{hendrickx2010semeval} created two sentence-level RE datasets by human annotation. However, these two datasets have a relatively small number of relation types and instances. 
The New York Times corpus \citep{sandhaus2008new} is another common relation extraction dataset used in the literature \citep{riedel-etal-2013-relation,nayak-ng-2019-effective}. It has been used for joint entity and relation extraction by \citep{nayak-ng-2020}. 
The large-scale TACRED~\citep{zhang-etal-2017-position} dataset is created based on the 2009--2014 TAC knowledge base population (KBP) challenges and crowd-sourced human annotations. FewRel~\citep{han2018fewrel} and FewRel 2.0~\citep{gao-etal-2019-fewrel} have been proposed to study the transferability and few-shot capability of RE models. However, early relation extraction datasets mainly focus on sentence-level RE, whereas many relations can only be expressed by multiple sentences.
The document-level relation extraction task has been proposed to build RE systems that are able to extract relations from multiple entities and sentences. \citet{yao2019docred} have created the DocRED dataset by distant supervision from Wikipedia articles and the Wikidata knowledge base. They sampled 5,053 documents for human annotation. The annotation strategy of DocRED is mainly based on machine recommendation and human filtering. With a similar approach, \citet{cheng-etal-2021-hacred} have created a Chinese document-level RE dataset that focuses on hard relation cases. 

\paragraph{Machine-Assisted Data Generation}
Since labeled data is expensive to obtain for complex NLP tasks, there are many research works on generating automatically labeled data. Distant supervision is first used by \citet{mintz2009distant} to generate relation extraction data without human efforts. 
Prior work on automatic data generation mainly relies on rule-based pattern matching \citep{lehmann2015dbpedia} and web crawling~\citep{buck2014n}. These types of rule-based methods are susceptible to noise propagation. With the rapid development of pre-trained language models~(PLMs; \citealp{devlin-etal-2019-bert}; \citealp{liu2019roberta} ; \citealp{brown2020language}), 
many recent works leverage PLMs for automatic data generation~(\citealp{10.1145/2433396.2433468}; \citealp{anaby2020not};  \citealp{zhou-etal-2022-melm}; \citealp{yang-etal-2020-generative}; \citealp{kumar-etal-2020-data}; \citealp{liu-etal-2021-mulda}). 
However, these methods typically depend on a certain set of supervised data. Another line of work utilizes manually designed prompts and instructions to generate data in an unsupervised manner~(\citealp{wang-etal-2019-tackling}; \citealp{schick-schutze-2021-generating}; \citealp{chia2022relationprompt}). Although these methods improve the performance on some downstream tasks, the quality of the machine-generated data still does not match human annotation. To mitigate noise from the machine-generated data, \citet{west2021symbolic}  generate a large amount of commonsense knowledge data and employ human annotators to filter the generated candidates. 

==> EMNLP_2022/sections/7_limitations.tex <==
\section{Limitations}
In this section, we discuss the limitations of our work. We have revised a popular document-level relation extraction dataset -- the DocRED dataset. We use an iterative human-in-the-loop approach for revising this dataset. However, after two rounds of annotation of the evaluation data, there might still be missing annotations, even though we have added almost twice the number of triples compared to the original DocRED dataset. That is, our re-annotation serves as a reasonable approximation to the ground truth, although it may still not be the gold standard for an ideal document-level RE scenario. We have provided a detailed analysis on annotation quality and comparison with contemporaneous work in Appendix~\ref{app:comparisonwithscratch}. The second limitation of our work is that human revision on the training data is only carried out in one round. The completeness level of the training data is lower compared to our evaluation data. Future research can focus on advanced algorithms for learning from imperfectly annotated data, which is actually very common in real applications. Nevertheless, such study still needs high-quality test data for reliable evaluation. 

\section{Ethical Considerations}
This paper focuses on revising the annotation on the false negative examples in the DocRED dataset, a publicly available and widely used benchmark for document-level relation extraction. All the documents and relations are provided in the original DocRED dataset. The annotators involved in this work were paid around 60 CNY per hour, which is more than three times the minimum wage in that area. The scope of this work is on revising the relation triples in these documents. However, there may be improper content within the Wikipedia articles themselves. The authors of this paper are not responsible for ethical issues arising from such improper Wikipedia content. 
